Design and construction of a Cherenkov imager for charge measurement of nuclear cosmic rays

A proximity focusing Cherenkov imager called CHERCAM, has been built for the charge measurement of nuclear cosmic rays with the CREAM instrument. It consists of a silica aerogel radiator plane across from a detector plane equipped with 1,600 1" diameter photomultipliers. The two planes are separated by a ring expansion gap. The Cherenkov light yield is proportional to the charge squared of the incident particle. The expected relative light collection accuracy is in the few percents range. It leads to an expected single element separation over the range of nuclear charge Z of main interest 1 < Z < 26. CHERCAM is designed to fly with the CREAM balloon experiment. The design of the instrument and the implemented technical solutions allowing its safe operation in high altitude conditions (radiations, low pressure, cold) are presented.

==> Makefile <==
FICHIER_TEX=chercam.tex
ARCHIVE=$(FICHIER_TEX:%.tex=%.zip)

all : 
	pdflatex ${FICHIER_TEX}
################################################
#lance le make de chaque sous rep
$(REP):
	@$(MAKE) -C $@ $(MAKECMDGOALS)

clean: $(REP)
	@echo "suppression des fichiers de compilation"
	@# fichiers de compilation latex
	@rm -f *.log *.aux *.dvi *.toc *.lot *.lof *.out
	@# fichiers de bibtex
	@rm -f *.bbl *.blg
	@# fichier zip 
	@rm -f *.zip

zip: 
	#rm ${ARCHIVE}
	grep includegraphics *.tex > liste.txt
	awk  '{st=index($$0,"{");rem=substr($$0,st+1); st=index(rem,"}"); rem=substr(rem,1,st-1); printf("zip -r ${ARCHIVE} %s.p*\nzip -r ${ARCHIVE} %s.j*\n",rem,rem);}' liste.txt > zip_liste.sh
	zip -r ${ARCHIVE} Makefile
	zip -r ${ARCHIVE} *.cls
	zip -r ${ARCHIVE} *.tex
	bash zip_liste.sh

cleaner: clean
	@echo "suppression des fichiers cibles"
	@rm -f ${FICHIERS_PDF}

